Adaptive Location Privacy with ALP

With the increasing amount of mobility data being collected on a daily basis by location-based services (LBSs) comes a new range of threats for users, related to the over-sharing of their location information. To deal with this issue, several location privacy protection mechanisms (LPPMs) have been proposed in the past years. However, each of these mechanisms comes with different configuration parameters that have a direct impact both on the privacy guarantees offered to the users and on the resulting utility of the protected data. In this context, it can be difficult for non-expert system designers to choose the appropriate configuration to use. Moreover, these mechanisms are generally configured once for all, which results in the same configuration for every protected piece of information. However, not all users have the same behaviour, and even the behaviour of a single user is likely to change over time. To address this issue, we present in this paper ALP, a new framework enabling the dynamic configuration of LPPMs. ALP can be used in two scenarios: (1) offline, where ALP enables a system designer to choose and automatically tune the most appropriate LPPM for the protection of a given dataset; (2) online, where ALP enables the user of a crowd sensing application to protect consecutive batches of her geolocated data by automatically tuning an existing LPPM to fulfil a set of privacy and utility objectives. We evaluate ALP on both scenarios with two real-life mobility datasets and two state-of-the-art LPPMs. Our experiments show that the adaptive LPPM configurations found by ALP outperform both in terms of privacy and utility a set of static configurations manually fixed by a system designer.

==> tex/system.tex <==
\section{\accio, a modular framework}\label{sec:system}

This section describes the different modules of the \accio workflow shown in Figure~\ref{fig:overview}. 
In \accio{}, the raw traces are protected using an LPPM (see Section~ \ref{sec:overview:LPPM}). Then, the protected traces are evaluated using a set of evaluators implementing privacy and utility metrics (see Section~\ref{sec:overview:evaluators}).  Finally, an optimizer iteratively modifies the configuration parameters of the LPPM to reach a set of specified privacy and utility objectives (see Section~\ref{sec:overview:optimizer}). The abstraction and components associated to these actions are detailed below.


\subsection{LPPM}\label{sec:overview:LPPM}

An LPPM is abstracted in \accio{} as an  operation taking a single raw mobility trace as input and producing the associated obfuscated trace.
It is hence a function $\mathcal{T} \rightarrow \mathcal{T}$.
Internally, LPPMs are implemented through a set of trace transformations. For instance, the \sonia{donner un example de comment Geo-I ou Promesse est modélisé dans accio car ça reste très abstrait.}
This component takes also as input configuration parameters associated to the considered LPPM.\sonia{attention: on dit que ça va de T vers T puis on dit que finalement ça prend d'autres parametres en entrée: ce n'est pas rigoureux. Il faut revoir la définition de la fonction.}


\subsection{Evaluators}\label{sec:overview:evaluators}

% TODO: talk about user-side metrics.
%TODO: integrate that somewhere.
%We have shown in~\cite{Mapomme14} that despite a high level of obfuscation, it is still possible to re-identify at least 63~\% of the users.
%It suggests that, while giving some formal bound about the level of privacy, these metrics are not very expressive about what an adversary can actually achieve with obfuscated data.
%Moreover, from a final user's point of view, we believe it would be more interesting and transparent to have a hint about an adversary potential power than some abstract $k$ or $\epsilon$ value.
%It would had more transparency to what protection mechanisms are good for, and raise awareness around privacy issues.

Similarly to~\cite{Shokri11,Mapomme14}, the evaluation component of \accio compares the output of some process when applied on a raw trace and on its obfuscated counterpart.
This comparison is done by what we call an evaluator, which produces a metric as output.
Formally, an evaluator $e \in \mathcal{E}$ is a function $\mathcal{T} \times \mathcal{T} \rightarrow \mathbb{R}$, which given a raw trace and an obfuscated trace outputs a single real value.
We do not make any assumption of this value's unit or meaning for now, it is up to the user to interpret it.
Note that we do not distinguish between privacy and utility metrics, mainly because some metrics can be viewed both as a privacy or utility metric.
The evaluation process, along with a definition of all implemented evaluators, is detailed in Section~\ref{sec:metrics}.

\subsection{Optimizer}\label{sec:overview:optimizer}

\accio does not only assess the effectiveness of the considered protection mechanism, 
but it is able to dynamically parametrise the LPPM with respect to some user-defined objectives in terms of privacy and utility.
%As shown in Figure \ref{fig:overview}, the optimizer exploits objectives to minimize or maximize metrics. 
As the framework does not distinguish between privacy and utility metrics, the choice to maximize or minimize is left to users.
The optimization process evaluates the current LPPM parametrisation and uses the metrics it obtains from evaluators to improve the configuration parameters.
This process is ran many times, and the best parametrisation is used to effectively obfuscate mobility traces before sending them to the LBS.
The optimization process is presented thoroughly in Section~\ref{sec:optimizer}.


%\subsection{Transformers}\label{sec:overview:transformers}
%Transformers are the components responsible for manipulating mobility traces.
%A transformer is an operation taking a single trace as input and producing zero, one or several traces.
%Thus, a transformer is a function $\mathcal{T} \rightarrow \mathcal{T}^n, n \in \mathbb{R}^+$.
%As transformers consume and produce traces, they can easily be composed.
%This allows us to abstract a large range of transformations, such as filtering, mapping, and splitting.
%
%Transformers are used during the preprocessing phase, which aims to prepare the raw mobility traces for the targeted application and use case.
%For example, in the online scenario, a navigation application requires the location information of users almost at real-time while a noise monitory crowd-sensing application requires information less frequently.
%In a similar manner, in the offline scenario, the data usually needs to be prepared, e.g., to remove noisy data, uniformise sampling rates or only keep records relevant to a specific period of time.

%\begin{itemize}
%  \item Filtering: when a transformer always produces either an empty list or a singleton containing the input trace.
%  \item Mapping: when a transformer always produces a singleton containing a modified version of the input trace.
%  \item Splitting: when a transformer produces a variable number of traces, whose union is the input trace.
%\end{itemize}

